Flexible Network Bandwidth and Latency Provisioning in the Datacenter

Predictably sharing the network is critical to achieving high utilization in the datacenter. Past work has focussed on providing bandwidth to endpoints, but often we want to allocate resources among multi-node services. In this paper, we present Parley, which provides service-centric minimum bandwidth guarantees, which can be composed hierarchically. Parley also supports service-centric weighted sharing of bandwidth in excess of these guarantees. Further, we show how to configure these policies so services can get low latencies even at high network load. We evaluate Parley on a multi-tiered oversubscribed network connecting 90 machines, each with a 10Gb/s network interface, and demonstrate that Parley is able to meet its goals.

==> README <==
The main tex file is eyeq++.tex, and you can follow
the other files from there:

\input{abstract}
\input{intro}
\input{motivation}
\input{relatedwork}
\input{design}
\input{latency}
\input{implementation}
\input{evaluation}
\input{conclusion}

To compile the PDF, just type "make"

After editing changes, commit your code by running:

  git commit -a -m "fix typos"

Repeat the above step until you've made all changes.

Then, just pull changes by running:

  git pull --rebase

And finally, push your changes:

  git push



==> evaluation.tex <==

\section{Evaluation}
\label{sec:evaluation}
We demonstrate that \sys achieves our goals of predictable bandwidth
sharing.

Since we built \sys on top of EyeQ, we refer the reader to
measurements in the EyeQ paper~\cite[\S5.1]{jeyakumar2013eyeq}.
\sys inherits EyeQ's results for: (i)~low CPU overhead when
compared to state-of-the-art software rate limiters;
(ii)  millisecond-timescale convergence times at the machine shapers.

The new aspects of \sys that we cover in this paper are:
\begin{itemize}
%  \item In the absence of rack/fabric brokers, we show that \sys is
%    able to gracefully degrade to per-receiver max-min fairness, even
%    in the presence of congestion within the network fabric.
  \item Rack brokers are highly efficient, and consumes less than 2ms
    wall-clock time to allocate bandwidth to as many as 100k services.
    The bandwidth overhead is less than 3Mb/s when rack broker
    interval is 1s.  Moreover, they converge to the fair rates within
    a few seconds.
  \item In an emulation, the fabric broker converges within 10s to
    limit the maximum bandwidth consumption across 100 racks.
  \item The rack broker can control the maximum utilization on the
    rackswitch, ensuring predictable tail latency for services in
    the rack, even in the presence of a malicious service that tries to
    grab all bandwidth.
  %\item Global fabric broker converges within 10s of seconds for high
  %  demands, and the racks default to.
\end{itemize}

{\bf Topology and parameters}: Unless otherwise noted, we use the
topology as shown in Figure~\ref{fig:topology}.  There are 10 hosts
under each of the 9 rackswitches.  Each host has a 10Gb/s NIC.
The network is oversubscribed 1:1.25 at the rackswitch.
We use the \sys parameters shown in Table~\ref{tab:parameters}.
\begin{table}[t]
\begin{center}
\begin{tabular}{ |p{0.25\textwidth}|r|r| }\hline
RCP aggressiveness & $\alpha$ & 0.5 \\\hline
RCP time interval & $T$ & 200$\mu$s \\\hline
Gain for EWHA & $\gamma$ & $\sfrac{1}{8}$ \\\hline
Rack broker frequency & $T_{\rm rack}$ & 1s \\\hline
Fabric broker frequency & $T_{\rm fabric}$ & 10s \\\hline
Rack broker timeout at machine broker & $T^t_{\rm rack}$ & 5s \\\hline
Fabric broker timeout at rack broker & $T^t_{\rm fabric}$ & 50s \\\hline
ECN marking threshold & & 80kB\\\hline
\end{tabular}
\end{center}
\caption{Parameters used in evaluating \sys.}\label{tab:parameters}\vspace{-4pt}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/topology}
\caption{{Topology of the testbed.  The network is oversubscribed by a
  factor of 1.25 (100Gb/s to 80Gb/s) at the
  rackswitch.}}\label{fig:topology}
\end{figure}

%\subsection{Microbenchmarks}

% We now evaluate aspects of the system that are unique to our work.
% Vimal: include this in the techreport.
\techreport{
\subsection{Machine shaper microbenchmarks}
{\bf Graceful degradation during network congestion}: The machine
shaper senses congestion when link utilization approaches capacity,
which is not sufficient if the network is congested.  Hence, the
machine shaper also uses ECN feedback from the network to back off
when links are congested.  We evaluate this scenario by having two
service instances under different racks send traffic to two their
respective receivers under the same rack, but on different machines.
We induce network congestion by disabling all but one link at the
receiving rackswitch, creating a 2-to-1 oversubscription at the
rackswitch.

Figure~\ref{fig:network-congestion} highlights an important point that
the machine shaper must operate at a fast enough timescale.  At time
t=0, only one service is active.  At t=40s, both services are active,
causing network congestion; therefore, bandwidth is shared almost
equally (Jain's Fairness Index is 0.99).  At time t=60s, we increased
$T$ from 200$\mu$s to 1ms; notice that the machine shaper is now too
slow to guarantee fair shares across receivers, as the transport layer
(TCP) also backs off due to network congestion.

If we were allowed to
change TCP to back off less aggressively, or to use UDP, a 1ms timescale
for reaction time would be sufficient.  We discuss the tradeoffs
between accurate and coarse-grained rate limiting and its impact on
flow completion times in~\S\ref{sec:lessons}.

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{graphs/network-congestion}
\caption{{When there is network congestion at the rackswitch, \sys
  gracefully falls back to a sharing model where receivers get
  (almost) equal shares of the network bottleneck link.
  \ignore{However, a
  fast reaction time ensures nearly ideal sharing.
  \fixthis{I don't think the figure actually demonstrates the
  last sentence in the caption.  Remove it?}}}}\label{fig:network-congestion}
\end{figure}
}

\ignore{
{\bf Rate limiter sharing}: \ignore{Sharing rate limiters without
  keeping per-source/destination requires less state, but at the
  expense of total utilization.}  Sender~`A' shares one rate limiter
to send TCP traffic to two receivers~B and C; receiver~B is allocated
a max = 1Gb/s, and receiver~C is allocated a max = 9Gb/s.  The shared
rate limiter aggregates feedback stream from both receivers using an
exponential weighted harmonic mean described
in~\S\ref{sec:sharing-rl}.  Table~\ref{tab:rl-sharing} shows the final
allocation and its split between the two receivers, as we vary the
number of TCP flows between A and B ($N_{A\rightarrow{}B}$), keeping
$N_{A\rightarrow{}C}$ fixed at 4.

\ignore{We see that though the rate limiter does not keep track of
  per-receiver splits, the total rate limit at A converges to a value
  such that the most bottlenecked receiver is not overwhelmed.}
\ignore{Since rate limiters will not be shared across jobs, any
  utilization loss is self-inflicted.}  \fixthis{(Jeff) There are
  several things I do not understand about this paragraph; we should
  talk about it.}

\begin{table}[h]\centering
\begin{tabular}{l|r|r|r|r}
$N_{A\rightarrow{}B}$            & 0 & 4 & 16 & 32 \\\hline
Total rate limit $R$~(Gb/s)   & 9.00 & 1.70  &   1.10  & 1.00 \\\hline
$A\rightarrow{}B$'s avg. share of $R$ & - & 0.85 &  0.90 & 0.99 \\
$A\rightarrow{}C$'s avg. share of $R$ & 9.00 & 0.85 &  0.20 & 0.01 \\
\end{tabular}
\caption{{Traffic from A to two receivers B and C share a
    single rate limiter, which, in a stateless fashion, ensures that
    capacities at both receivers are not violated.}}
\label{tab:rl-sharing}
\end{table}

We vary the number of TCP flows between A and B
($N_{A\rightarrow{}B}$), keeping $N_{A\rightarrow{}C}=4$.  In all
cases, B does not receive more traffic than its allowed maximum of
1Gb/s.  However, when $N_{A\rightarrow{}B}=0$, $A\rightarrow{}C$ is
able to send at 9Gb/s to C.}

% C1=1Gb/s, C2=10Gb/s

% vary number of flows

\subsection{Microbenchmarks for Rack and Fabric brokers}
{\bf Bandwidth overhead}: In our rack broker implementation,
each machine broadcasts its own service utilizations to other machines
under the rack.  Each service can be represented as a 4B integer, and
its utilization as another 4B floating point number.  At 8B per
service, even 1000 bandwidth-intensive services in a rack would
generate only 8KB of data, plus some overhead for packet headers.
If there are 40
machines in a rack, unicasting this data to each machine once/sec
would cost less than 3Mb/s per machine.

{\bf Computation overhead}: The rack broker repeatedly computes
hierarchical max-min shares among $N$ services.
Table~\ref{tab:rackshaper-compute} shows the wall-clock time
%\fixthis{don't say ``cost''; say ``CPU time'' or ``wall-clock time''.}
of computing these
shares for a single level in a hierarchy, for various values of $N$
(using one core of a 2.4GHz Linux desktop machine).  We initialized
demands randomly such that the load is close to the capacity.  Note
that the
wall-clock time
of the `waterfill' algorithm scales well
with $N$, as every iteration of the waterfill satisfies the demand for
at least one service.  In practice, every iteration often satisfies
the demand for more than one service.

\begin{table}[h]\centering
\begin{tabular}{l|r|r|r|r}
$N$   & 100     & 1k       & 10k       & 100k \\\hline
Time  & 2$\mu$s & 12$\mu$s & 320$\mu$s & 1.6ms
\end{tabular}
\caption{Average wall-clock time per iteration of max-min share computation.}
\label{tab:rackshaper-compute}
\end{table}

{\bf Convergence speed}: The hierarchical max-min algorithm converges
in \emph{one invocation}, and therefore the convergence speed only
depends on the speed of exchanging information and the computation
time.  The rack broker can also work at the rate of 10 times per
second, consuming 30Mb/s bandwidth, converging to the allocations in
100ms.  In practice, however, we found 1s time granularity to be
sufficient in ensuring isolation, as the machine shaper works at
faster timescales to ensure the network does not experience persistent
congestion.

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{graphs/fabric-broker-util-both.pdf}
\caption{{\normalsize At t=0, we start the fabric broker, and it takes 10s
    for it to take effect. However, once the fabric broker starts to
    allocate bandwidth, it converges within a few iterations (at
    t=30s) and limits the tenant's usage to $<$20Mb/s, despite its
    bursty traffic pattern.  We change the limit to 50Mb/s, 100Mb/s,
    150Mb/s, 20Mb/s and back to 100Mb/s every 50s to illustrate
    convergence.}}\label{fig:fabric-broker}%\vspace{-1em}
% scripts, graphs, and data in /Users/jvimal/proj/eyeq++/mn-burst
\end{figure}

{\bf Fabric broker}: To test the convergence of the fabric broker at
large scale, we emulated a 100 rack cluster in
Mininet~\cite{handigol2012reproducible} with one tenant that is rate
limited to 20Mb/s.  Each rack has a 100Mb/s link to the fabric; it
picks another rack at random and sends a UDP data burst for 5s, and
sleeps for another 2s until t=300s (onoff).  In another experiment,
the traffic is less bursty (steady): it does not sleep for 2s, but
instead, it immediately sends traffic to another random rack.  The
burst time is smaller than the 10s interval at which the racks
communicate with the fabric broker.  Figure~\ref{fig:fabric-broker}
shows the time series of the aggregate utilization of the tenant: as
we can see, the fabric broker converges after the first burst, and
within a few iterations, the tenant is limited to its 20Mb/s.  In
practice, the rack broker will ensure the initial burst does not
adversely affect the performance of other services within the rack.
\highlight{This global service limit would not be feasible with proposals such as
EyeQ/ElasticSwitch, as the service's per-rack limit depends on
bandwidth usages of other racks.}

%% \subsubsection{Fabric shaper}
%% {\bf Bandwidth overhead}

%% {\bf Computation overhead}

%% {\bf Convergence speed}

\subsection{Macrobenchmarks}\label{subsec:macro}
{\bf Policy}: We demonstrate how \sys can
protect the rackswitch links from persistent congestion.  On each
machine in the topology, we
instantiate two service endpoints A and B, each of which is given equal
bandwidth at the machine level.  At the rack uplink, service A is
given at most 30Gb/s,
% of the rackswitch capacity to the fabric,
and service B is
given at least 30Gb/s, but the peak load on the rack is limited to 60Gb/s.  Recall that \sys's final
allocation depends on the most constrained resource.

{\bf Throughput protection}: One of the racks is designated as the
receiver.  The traffic pattern consists of long-lived transfers
between every pair of sender and receiver (a full mesh).
Figure~\ref{fig:rackswitch} shows the utilization of each
service at the receiving rackswitch.  At the start of the
experiment, only service A is active; notice that it uses only
30Gb/s.  At about T=300s,
%\fixthis{how about ``At $T=250$'' or whatever the correct value is?},
we start service B, which
takes around 50s to ramp up.  \sys converges faster than the time it
takes for all flows of service B to ramp up, but by the time all flows
are running at full line rate, service B is able to utilize its full
30Gb/s link capacity.  When service A finishes, service B is able to
utilize all the remaining capacity up to 60Gb/s.
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{graphs/rackswitch-longlived}
\caption{{Two services A and B sharing limited rackswitch capacity.
  Service A can consume at most 30Gb/s, while service B can consume at
  least 30Gb/s but the total is limited to 60Gb/s.  The utilization data is obtained
  every second, and the plot marks are every 30s.
  %\remark{Do the plot marks actually add any value? maybe remove them.}
  % Vimal: they help when printed in black and white
  }}\label{fig:rackswitch}
\end{figure}

{\bf Latency protection}: Using the same policy as above, we show how
\sys can protect the latency of a service against high-rate adversarial
traffic.
% provide latency protection to a service protecting against an
% adversarial traffic that offers high load.
We run the same
configuration as above, and both services mimic a client-server
workload with all-to-all communication between senders spread
across all but one rack, and receivers in the one remaining rack.
There are 24
TCP connections between each (service,machine) pair.

Service A uses 200kB RPCs such that its total offered load is 14\% of
the receivers' rackswitch capacity.  Service B uses 1MB RPCs such that
the \emph{total offered load} on the rackswitch is 15\%, 50\%, 70\% and
$>$100\%.  Table~\ref{tab:latency} shows the 99th percentile
% latency
FCT
of 200kB RPCs, while we varied the total load at the rackswitch.  The
mean RPC inter-arrival time $t_{\mu}$ is chosen to match the load, and
the inter-arrivals are sampled uniformly at random between 0 and
$2t_{\mu}$.  The 99th percentile FCT is computed after running for 20
minutes.  \ignore{Note that the total utilization at the rackswitch is limited
to 80\% of its capacity.}

The results in Table~\ref{tab:latency} show, not surprisingly,
that \sys does not significantly affect latency at offered loads
below 100\%.
The table also shows that service A's latency increases with the total
offered load, even though A's offered load is constant, since it
is sharing contention points with service B.  Therefore, one
must assume that B is fully utilizing its maximum bandwidth
allocation when deriving a tail-latency bound for A.

These results also demonstrate that without \sys, the tail
latency of service A can become very large when B tries to
increase its load past its allocated capacity, but \sys protects A's
tail latency.  Naturally, B's own tail latency becomes unbounded when
its load exceeds its guaranteed bandwidth.
Since the oversubscription is at the receiving rackswitch, and the load is
uniformly spread across machines under that switch, \sys's protection is
primarily due to the rack broker's allocations.

\ignore{
To summarize our findings:
%\begin{itemize}
(1) Not surprisingly, the latency difference with and without \sys is
not substantial at loads where the offered load on the network is
anything less than 100\%.

(2) Service A's load is constant but its latency increases with the
total load as it shares the network queues with service B, and hence
is affected by B's load.  Thus, any guarantees on A's tail latency
will have to be made assuming B is fully utilizing its bandwidth
share.

(3) \sys is responsive and protects the latency sensitive service,
when service B tries to exceed its fair bandwidth share.  Naturally,
service B's tail latency will grow unbounded since its load is more
than its guaranteed bandwidth.

(4) Since the oversubscription is at the rackswitch, and the load is
uniformly spread across machines under the rack, \sys's protection is
primarily due to the rack broker's allocations.
}

\begin{table}[t]\centering
\vspace{-2em}
\begin{tabular}{l|r|r|r|r}
 & \multicolumn{4}{c}{Total offered load at receiver rackswitch} \\
\cline{2-5}
%Off. Load $\rightarrow$
 &  15\%    & 50\%       & 70\% & $>100$\%   \\\hline
%Util \%   & 15\% & 50\%  & 70\%  & 80\% \\\hline
%Util. (w/o) & 12Gb/s & 40Gb/s &  & - \\\hline
A (w/o) & 2.46ms & 3.03ms & 6.04ms &       \red{\bf 1094.15ms}              \\\hline
B (w/o) & 6.75ms & 6.29ms & 13.21ms &      -               \\\hline\hline
%Util. (with) & 12Gb/s & 40Gb/s & 56Gb/s & 72Gb/s \\\hline
A (with)  & 2.22ms & 2.83ms & 6.11ms &     32.40ms     \\\hline
\blue{A (bounds)} & \blue{9.01ms} & \blue{15.32ms} & \blue{25.53ms} & \blue{38.30ms} \\\hline
B (with)  & 6.72ms & 6.30ms & 13.52ms &    -       \\
\end{tabular}
\caption{{The 99th percentile RPC completion time, as a
    function of the total load offered at the receiver rackswitch,
    with and without (w/o) \sys.  The bounds on tail latency are
    computed using equation~\ref{eqn:result}.  As indicated in
    boldface, the latency without \sys suffers at high utilization.}}\vspace{-1.5em}
\label{tab:latency}
\end{table}

%(5)
The total load at the rackswitch was limited to 60Gb/s (or about 80\%
of its capacity).  For this experiment, the machine shaper iterates
every 500$\mu$s to recompute $R(t)$, and it converges (in the worst
case) to within 30 iterations, to allocations within 0.01\% of the
ideal rate, regardless of the number of
flows~\cite{jeyakumar2013eyeq}.  In practice, we found that 15
iterations suffice.  Thus, the burst size $\sigma$ can be bounded and
is dominated by the convergence time of the congestion control
algorithm.  Table~\ref{tab:latency} also shows the bounds on the flow
completion time computed using Equation~\ref{eqn:result}.  As we can
see, the bounds are useful indicators of performance at high load.
The bounds are a bit pessimistic at lower loads as the bounds are
calculated making no assumptions on the arrival process; with more
assumptions, they can be improved further.

%, we can see that the the
%\emph{worst-case} flow completion time ${\rm FCT}(f)$ for service A's
%200kB flows is bounded by

%% {
%% \begin{align*}
%% {\rm FCT}(f) & \leq \frac{\sigma+Z(f)}{C(1-\rho)} \\
%%              & = \frac{10~\text{Gb/s}\times500~\mu{}\text{s}\times{}15 + 200~\text{kB}}{10~\text{Gb/s}\times(1-0.8)}\\
%%              & = 38.30~\text{ms}
%% \end{align*}}%

%%      \noindent which is close to the 99th percentile FCT shown
%%      in Table~\ref{tab:latency}. (We do not
%%      bound %\remark{``we do not bound''?}
%%      the maximum FCT, as other factors such as TCP timeouts
%%      and OS scheduling can have a noticeable impact on the maximum
%%      FCT.)
\highlight{If services A and B are work-conserving,
they will saturate the rackswitch uplink, congesting the network fabric,
causing overload at contention point~(iii) in Figure~\ref{fig:contention}.
Since this scenario violates the assumptions of a congestion-free network core
made in EyeQ, it will be ineffective in controlling tail latency.
EyeQ will default to a TCP-like behavior, thus
service A's tail latency will be as large
as shown in Table~\ref{tab:latency} in bold/red.
EyeQ worked around this
issue by doing admission control on service instances, ensuring
the rack bandwidth is never over-committed.  This means that peak load at the
rackswitch can be controlled only using non work-conserving
allocations, by capping each
of the ten instances of service A and service B to 3Gb/s, so the total
allocated capacity is 60Gb/s. Though
EyeQ supports non work-conserving allocations, static
reservation wastes as much as
\emph{half the rack's network capacity}---if one of
the services is inactive.  Hence, we need a mechanism to dynamically
adjust each service's allocations, which is exactly what \sys
implements.}

  %\item Note that the 99th percentile latency for the antagonist service B
  %  is worse than what it could be without any protection!  Naturally,
  %  one might suspect \sys's overheads being a reason for this.
  %  However, we will show in the next section that latency increase is
  % \emph{fundamental} to the specific bandwidth sharing model.
  %\item Interestingly, we were able to sustain higher utilizations
  %  with \sys, at higher offered loads on the network.
%\end{itemize}

%It is important to note that \sys's protection takes effect only in
%extreme conditions where malicious or buggy services try to grab a
%disproportionate share of network bandwidth.

%% At much higher loads ($>$80\%), high latency is fundamentally
%% inevitable unless flows are prioritized.  In fact, in most cases
%% (except in case of bulk data copies) application-level traffic is
%% inherently closed loop, and elastic.  For instance, RPCs may be issued
%% to multiple service replicas and slow responses will timed
%% out~\cite{jalapartispeeding} to meet application SLA requirements.
%% Thus, the maximum utilization we see at rackswitches typically doesn't
%% exceed a threshold (70--80\%) of the rackswitch capacity, beyond which
%% the utilization has a noticeable impact on the application SLA.

%% For instance, since the offered load of service A is less than its
%% bandwidth, we could simply prioritize service A over service B at all network
%% hops.  We found that its latency was the same as its latency at 15\%
%% load, since none of service A's packets contend with service B's packets.
%% However, due to strict prioritization, we found that service B's latency
%% shot up to XX.

%{\bf Closed loop load test}:

\section{Discussion}\label{sec:lessons}
{\bf Timescales for traffic shaping}:
As the authors of EyeQ noted~\cite[\S2.2]{jeyakumar2013eyeq}, rate
control must be fast enough to react before queues build up and increase
latency for competing flows.  However, we also found that such fast
and accurate rate control can also hurt the completion times of RPC
transfers.
(This insight is not specific to \sys, but applies to any
bandwidth management scheme targeted at an environment
with relatively high bandwidth and low latency.)

\begin{figure}[t]
\centering
\includegraphics[width=0.40\textwidth]{figures/limit-nolimit}
\caption{{To rate limit or not to rate limit: Rate limiting and
  accurate pacing improves sharing, but also increases RPC completion
  times.}}\label{fig:limit-nolimit}\vspace{-3pt}
\end{figure}

To understand this, consider the scenario in
Figure~\ref{fig:limit-nolimit}, where service receives three 2.5MB RPCs
at the same time, and then waits for 10ms; thus, its demand
oscillates between 0 and 6Gb/s (measured over 10ms)
%\remark{this said ``20ms'' but that seemed wrong})
every 20ms.
Suppose our policy limits the service to 3Gb/s; over a period of
20ms, its usage complies with the policy.  However, over a 10ms
interval (e.g., from 0--10ms), the service temporarily exceeds its
allocation by 3Gb/s.

If we use a fast-acting rate-control mechanism,
the service is always precisely rate limited,
so demand from 0--10ms spills over to the next
interval.  This means that all RPCs take 20ms to finish.
If, however, the service is not rate-limited at all, all of
its RPCs will finish in 10ms, thus halving the maximum
completion time.
This highlights a fundamental
tradeoff between accurate rate guarantees and RPC completion times.
However, it is difficult to pick a specific upper bound for the 
rate-limiting burst size,
as the example in Figure~\ref{fig:limit-nolimit}
still holds if RPC sizes (and timescales) are scaled up by a factor of
10.

Thus, at the machine shaper, the service rate limiters should have a
configurable burst size for coarse-grained rate limiting, and rate
meters should have a configurable time interval to measure ingress
utilizations.  In
general, the burst size of a latency-sensitive service should be
higher than a collocated throughput-sensitive service.  This burst
size approach is a special case of the more general \emph{fair service
  curves}~\cite{stoica1997hierarchical},
% discussed in literature, which is 
an approach to decouple rate guarantees from delay guarantees.  A rule
of thumb is to set burst sizes larger than the size of flows that are
low-latency.

{\bf Tighter latency bounds}: The latency bound shown in
Equation~\ref{eqn:result} depends both on the capacity $C$ and on the
total load $\rho$ on the network queues, and increases steeply as load
increases (i.e. as $\rho\rightarrow 1$).  Thus, if the resulting
latency bounds are unacceptable, either (a) low-latency RPCs must not
be exposed to load offered by other services, which can be achieved by
coarse-grained prioritization, or (b) network capacity should be
increased.  \sys helps in two ways: (i) it can control the peak
utilization at the rack uplinks/downlinks regardless of the number of
service endpoints under the rack; (ii) \sys serves as a useful
monitoring and protection mechanism for buggy services that might
consume more bandwidth than what is specified according to a policy.
\ignore{
\remark{I don't understand this; how does \sys provide any more
  protection than simply rate-limiting these buggy services according
  to their policy's max limit?  Vimal: rate limiting (at the rack
  level) is the important point here.  By limiting bandwidth
  consumption at the rack, you can use Eqn 2 to bound the tail
  latency.}}

%{\bf When do we actually \sys?}: Almost all prior work focused stress
%evaluated their works in the worst case when there are heavy bandwidth
%consumers saturating the network all time.

%% The example helps realize the importance of relaxing the granularity
%% of rate limiting for latency sensitive services.  We did notice that a
%% higher burst size reduced the 99th percentile RPC latency in our
%% experiments by as much as 10x.  We used a burst interval of 500$\mu$s
%% for the rate limiter and rate meter so the rate limiters do not
%% aggressively pace packets, so RPCs that are smaller than 500kB
%% (500$\mu$s burst at 10Gb/s) can benefit.

%% {\bf Latency}:
%% burst size.


==> intro.tex <==
\section{Introduction}\label{sec:intro}
Multi-tenancy is inevitable at large scale.  In a large scale
datacenter, we see on average 10s of jobs per server.  A typical
server is shared by the following applications that have diverse
performance requirements from the network:

\begin{itemize}
  \item {\bf Bandwidth Intensive}: A MapReduce job during its read and
    shuffle stages, and large file copies.
  \item {\bf Latency Sensitive}: The frontend for user-facing
    services, such as web search.
  \item {\bf Bandwidth and Latency Sensitive}: Infrastructure services
    such the distributed file system (DFS), have a mix of bandwidth
    and latency sensitive flows.
  \item {\bf Adversarial}: External customer virtual machines (VMs),
    in public clouds such as Amazon EC2, Windows Azure.
\end{itemize}

Prior work~(see~\cite{mogul2012we} for a detailed summary) in this
space has already made the case for sharing bandwidth across entities
that are less granular than a TCP flow.  As an example,
Oktopus~\cite{ballani2011towards},
Gatekeeper~\cite{rodrigues2011gatekeeper},
EyeQ~\cite{jeyakumar2013eyeq} and
ElasticSwitch~\cite{popa2013elasticswitch} all provide the notion of a
dedicated physical network (of a specified per-endpoint capacity) to a
tenant owning a collection of VMs spread across the datacenter.  This
specific notion of sharing is useful in a cloud setting where the
motive is to sell bandwidth to external customers.  This policy can be
realized under an important constraint that the VM placement must
satisfy all bandwidth guarantees in the \emph{worst case} when all VMs
are active simultaneously.

However, additional practical requirements require us to rethink how
these proposals should actually be deployed.  For instance, not all
services need such strong bandwidth guarantees.  In such cases,
network oversubscription plays a role in sharing bandwidth.  As an
example, the infrastructure operator should be able to specify that
(say) free-tier VMs in a rack should be allocated at most 10\% of the
rackswitch uplink and downlink, regardless of the number of such VMs
under the rack.

To our knowledge, none of the recent proposals allow us to specify and
enforce flexible bandwidth sharing policies other than bandwidth
guarantees, which limits their applicability.  Also, prior work does
not talk about provisioning bandwidth in light of a service's latency
requirements.  \emph{Our work endeavors to support richer policies,
  and shows that carefully provisioning capacity leads to low tail
  latency.}  Specifically, a service policy specifies a guaranteed
minimum bandwidth, a maximum limit, and a weight, for sharing
bandwidth at key contention points in the network.  The weight
parameter ensures that any excess bandwidth is shared between services
in the ratio of their weights.  Service policies can also be nested.
An explicit policy means that the applications can expect network
performance that is easily predictable.  Figure~\ref{fig:example}
shows an example of such a policy at the machine and the top-of-rack
switch (rackswitch).

%% To this end, we present \sys, an end-to-end bandwidth management
%% system for intra-datacenter traffic.  \sys supports a
%% \emph{hierarchical sharing policy} (Figure~\ref{fig:example}) to share
%% datacenter bandwidth at the key points of contention: a service (or
%% groups of services) gets a min, or max, or weighted share of machine
%% bandwidth, or rackswitch bandwidth, or global fabric bandwidth.  The
%% policies encode constraints on bandwidth allocations, and the final
%% allocation therefore depends on the most constraining policy.

We do not dismiss prior work.  Our main contribution is to show how we
can leverage them in a \emph{systematic fashion} to realize other
useful sharing objectives.  We build on top of the open-sourced
project, EyeQ, and refer to our system as \sys.  The roots of our
design lie in specifying the sharing objective explicitly and then
using optimization-decomposition to decompose the global problem into
manageable subproblems~\cite{palomar2006tutorial}.

%The
%hierarchical model is flexible enough to capture isolation
%inter-service isolation as well.  We show how this hierarchical
%allocation

%With \sys,
%an operator would be able to specify that MapReduce jobs should get at
%least 10\% of the machine bandwidth, at least 30\% of the rackswitch
%capacity, and at most 50\% of the fabric bandwidth, regardless of
%other services in the system.

\begin{figure}[t]
  \centering\includegraphics[width=0.4\textwidth]{figures/example-2.pdf}
  \caption{\sys's supports a hierarchical sharing policy.  The top
    figure shows the service placement on machines under the rack of a
    given capacity, and the bottom half illustrates sharing policies
    at the machine and rack.}\label{fig:example}
\end{figure}

At the core of \sys is a bandwidth broker that allocates capacities to
services in a hierarchical fashion.  At the lowest level, each VM (or
job, or service) on a machine is allocated a transmit and receive
capacity that is periodically adjusted by the bandwidth broker, based
on (i) machine level utilization (\S\ref{subsec:machineshaper}), (ii)
rackswitch level utilization (\S\ref{subsec:rackbroker}), and (iii)
fabric utilization (\S\ref{subsec:fabricbroker}).  Rate enforcement on
each VM is done in the \emph{dataplane} by EyeQ.\ignore{EyeQ uses
  per-destination rate limiters at senders that coordinate with
  receivers using feedback messages to enforce the hose-model in an
  end-to-end fashion.}  An example policy to share rack bandwidth is
shown in Figure~\ref{fig:example}, where the rackswitch broker
allocates DFS at least 6Gb/s, and atmost 8Gb/s, and VMs a maximum of
1Gb/s.  The VM's 1Gb/s rack bandwidth is inturn shared in a `weighted
max-min'~\cite[Sec.~6.5.2]{bertsekas1992data} fashion among VMs in the rack.  By decomposing the global
sharing objective into rack and machine sub-problems, we are able to
scale the system to a large datacenter.

The remainder of the paper discusses each component in more detail: In
\S\ref{sec:background}, we outline the main requirements based on
observations from production datacenters.  In \S\ref{sec:design}, we
explicitly state our sharing objective, our algorithm to compute
bandwidth shares, and show that these guarantees are useful predictors
of latency in \S\ref{sec:latency}, followed by the implementation in
\S\ref{sec:implementation}.  We conclude with a large scale evaluation
in \S\ref{sec:evaluation} of \sys in a real cluster of 90 machines.

%% {\bf What about latency guarantees?}  In general, latency guarantees
%% can be specified on a per-packet (e.g., the end-to-end delay of a
%% packet is $<$~1ms), or at an RPC-level (e.g., the 95th percentile of
%% request completion times is $<$~10ms).  Achieving latency guarantees
%% is fundamentally difficult due to the stochastic nature of flow
%% arrivals which have to be precisely quantified and modeled to offer
%% any reasonable guarantees.  Moreover, the low-latency nature of
%% datacenter applications require require careful engineering of other
%% aspects of the system, such as kernel thread scheduling~\cite{},
%% memory isolation~\cite{}, etc., which is beyond the scope of this
%% paper.  Fortunately, as we will show, the bandwidth given to a service
%% \emph{bounds} the tail of the latency distribution as long as the
%% service arrivals and job sizes can be described precisely.

%% {\bf What about inter-datacenter traffic?}  \sys does not explicitly
%% handle inter-cluster traffic.  Instead, inter-cluster bandwidth
%% management is delegated to the Bandwidth Enforcer system described
%% in~\ref{}.

